A new calibration for the Blue Horizontal Branch

We suggest a simple analytic approximation for magnitudes and hence distances of Blue Horizontal Branch (BHB) stars in Sloan colours. Precedent formulations do not offer a simple closed formula, nor do they cover the full dependences, e.g. on metallicity. Further, using BHB star samples from the Sloan Digital Sky Survey (SDSS) we validate our distance calibration directly on field stars instead of globular clusters and assess the performance of other available distance calibrations. Our method to statistically measure distances is sufficiently accurate to measure the colour and metallicity dependence on our sample and can be applied to other sets of stars or filters.

==> PaxHeader/Fermani_Schoenrich_a.tex <==
18 uid=2099829945
20 ctime=1357748082
20 atime=1357748082
38 LIBARCHIVE.creationtime=1356026929
24 SCHILY.dev=771751941
24 SCHILY.ino=145314812
18 SCHILY.nlink=1

